BEAS: Blockchain Enabled Asynchronous & Secure Federated Machine Learning

Federated Learning (FL) enables multiple parties to distributively train a ML model without revealing their private datasets. However, it assumes trust in the centralized aggregator which stores and aggregates model updates. This makes it prone to gradient tampering and privacy leakage by a malicious aggregator. Malicious parties can also introduce backdoors into the joint model by poisoning the training data or model gradients. To address these issues, we present BEAS, the first blockchain-based framework for N-party FL that provides strict privacy guarantees of training data using gradient pruning (showing improved differential privacy compared to existing noise and clipping based techniques). Anomaly detection protocols are used to minimize the risk of data-poisoning attacks, along with gradient pruning that is further used to limit the efficacy of model-poisoning attacks. We also define a novel protocol to prevent premature convergence in heterogeneous learning environments. We perform extensive experiments on multiple datasets with promising results: BEAS successfully prevents privacy leakage from dataset reconstruction attacks, and minimizes the efficacy of poisoning attacks. Moreover, it achieves an accuracy similar to centralized frameworks, and its communication and computation overheads scale linearly with the number of participants.

==> figure/backdoor-acc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color2}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}
\definecolor{color3}{rgb}{0.505882352941176,0.447058823529412,0.698039215686274}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=None, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=none},
tick align=outside,
tick pos=both,
x grid style={white!80!black},
xlabel={Global Round (s)},
xmajorgrids,
xmin=0, xmax=55,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.4, ymax=0.6,
ytick style={color=white!15!black}
]
\addplot [thick, color0]
table {%
0 0.510869562625885
1 0.505434811115265
2 0.489130437374115
3 0.505434811115265
4 0.507246375083923
5 0.489130437374115
6 0.489130437374115
7 0.490942031145096
8 0.47826087474823
9 0.498188406229019
10 0.474637687206268
11 0.476449280977249
12 0.489130437374115
13 0.489130437374115
14 0.498188406229019
15 0.503623187541962
16 0.498188406229019
17 0.5
18 0.507246375083923
19 0.528985500335693
20 0.505434811115265
21 0.501811623573303
22 0.5
23 0.505434811115265
24 0.510869562625885
25 0.501811623573303
26 0.503623187541962
27 0.510869562625885
28 0.503623187541962
29 0.519927561283112
30 0.523550748825073
31 0.510869562625885
32 0.536231875419617
33 0.498188406229019
34 0.512681186199188
35 0.501811623573303
36 0.503623187541962
37 0.51630437374115
38 0.505434811115265
39 0.519927561283112
40 0.527173936367035
41 0.501811623573303
42 0.541666686534882
43 0.567028999328613
44 0.568840563297272
45 0.58152174949646
46 0.539855062961578
47 0.579710125923157
48 0.572463750839233
49 0.532608687877655
50 0.51630437374115
51 0.501811623573303
52 0.536231875419617
53 0.525362312793732
};
\addlegendentry{BEAS Backdoor}
\addplot [thick, color1]
table {%
0 0.510869562625885
1 0.510869562625885
2 0.489130437374115
3 0.510869562625885
4 0.498188406229019
5 0.487318843603134
6 0.483695656061172
7 0.485507249832153
8 0.492753624916077
9 0.494565218687057
10 0.485507249832153
11 0.494565218687057
12 0.483695656061172
13 0.490942031145096
14 0.481884062290192
15 0.489130437374115
16 0.480072468519211
17 0.480072468519211
18 0.489130437374115
19 0.489130437374115
20 0.5
21 0.498188406229019
22 0.505434811115265
23 0.509057998657227
24 0.509057998657227
25 0.505434811115265
26 0.51630437374115
27 0.507246375083923
28 0.501811623573303
29 0.509057998657227
30 0.510869562625885
31 0.514492750167847
32 0.501811623573303
33 0.501811623573303
34 0.501811623573303
35 0.509057998657227
36 0.509057998657227
37 0.505434811115265
38 0.503623187541962
39 0.505434811115265
40 0.503623187541962
41 0.509057998657227
42 0.525362312793732
43 0.532608687877655
44 0.510869562625885
45 0.545289874076843
46 0.512681186199188
47 0.509057998657227
48 0.512681186199188
49 0.505434811115265
50 0.505434811115265
51 0.505434811115265
52 0.51630437374115
53 0.514492750167847
};
\addlegendentry{BEAS Backdoor with Noise (0.10)}
\addplot [thick, color2]
table {%
0 0.510869562625885
1 0.507246375083923
2 0.489130437374115
3 0.492753624916077
4 0.510869562625885
5 0.490942031145096
6 0.487318843603134
7 0.483695656061172
8 0.47826087474823
9 0.483695656061172
10 0.492753624916077
11 0.5
12 0.501811623573303
13 0.485507249832153
14 0.476449280977249
15 0.472826093435287
16 0.476449280977249
17 0.485507249832153
18 0.483695656061172
19 0.489130437374115
20 0.518115937709808
21 0.52173912525177
22 0.52173912525177
23 0.518115937709808
24 0.519927561283112
25 0.507246375083923
26 0.530797123908997
27 0.528985500335693
28 0.519927561283112
29 0.534420311450958
30 0.547101438045502
31 0.51630437374115
32 0.512681186199188
33 0.509057998657227
34 0.532608687877655
35 0.518115937709808
36 0.539855062961578
37 0.507246375083923
38 0.51630437374115
39 0.518115937709808
40 0.523550748825073
41 0.523550748825073
42 0.58695650100708
43 0.532608687877655
44 0.532608687877655
45 0.530797123908997
46 0.536231875419617
47 0.554347813129425
48 0.512681186199188
49 0.561594188213348
50 0.505434811115265
51 0.501811623573303
52 0.53804349899292
53 0.545289874076843
};
\addlegendentry{BEAS Backdoor Clip Val (0.60)}
\addplot [thick, color3]
table {%
0 0.510869562625885
1 0.489130437374115
2 0.489130437374115
3 0.489130437374115
4 0.510869562625885
5 0.492753624916077
6 0.492753624916077
7 0.505434811115265
8 0.507246375083923
9 0.510869562625885
10 0.505434811115265
11 0.503623187541962
12 0.505434811115265
13 0.505434811115265
14 0.505434811115265
15 0.507246375083923
16 0.505434811115265
17 0.503623187541962
18 0.509057998657227
19 0.505434811115265
20 0.507246375083923
21 0.5
22 0.489130437374115
23 0.494565218687057
24 0.481884062290192
25 0.496376812458038
26 0.476449280977249
27 0.492753624916077
28 0.5
29 0.465579718351364
30 0.505434811115265
31 0.476449280977249
32 0.494565218687057
33 0.472826093435287
34 0.474637687206268
35 0.480072468519211
36 0.476449280977249
37 0.467391312122345
38 0.474637687206268
39 0.463768124580383
40 0.483695656061172
41 0.483695656061172
42 0.480072468519211
43 0.496376812458038
44 0.467391312122345
45 0.490942031145096
46 0.487318843603134
47 0.476449280977249
48 0.498188406229019
49 0.476449280977249
50 0.507246375083923
51 0.501811623573303
52 0.496376812458038
53 0.494565218687057
};
\addlegendentry{BEAS with Prune Sparcity (0.50)}
\end{axis}

\end{tikzpicture}


==> figure/krum-graph.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color2}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=None, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=none},
tick align=outside,
tick pos=both,
x grid style={white!80!black},
xlabel={Global Round (s)},
xmajorgrids,
xmin=0, xmax=55,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.5, ymax=1,
ytick style={color=white!15!black}
]
\addplot [thick, color0]
table {%
0 0.955353915691376
1 0.955353915691376
2 0.955353915691376
3 0.955353915691376
4 0.955353915691376
5 0.955353915691376
6 0.955353915691376
7 0.955353915691376
8 0.955353915691376
9 0.955353915691376
10 0.955353915691376
11 0.955353915691376
12 0.955353915691376
13 0.955353915691376
14 0.955353915691376
15 0.955353915691376
16 0.955353915691376
17 0.955353915691376
18 0.955353915691376
19 0.955353915691376
20 0.955353915691376
21 0.955353915691376
22 0.955353915691376
23 0.955353915691376
24 0.955353915691376
25 0.955353915691376
26 0.955353915691376
27 0.955353915691376
28 0.955353915691376
29 0.955353915691376
30 0.955353915691376
31 0.955353915691376
32 0.955353915691376
33 0.955353915691376
34 0.955353915691376
35 0.955353915691376
36 0.955353915691376
37 0.955353915691376
38 0.955353915691376
39 0.955353915691376
40 0.955353915691376
41 0.955353915691376
42 0.955353915691376
43 0.955353915691376
44 0.955353915691376
45 0.955353915691376
46 0.955353915691376
47 0.955353915691376
48 0.955353915691376
49 0.955353915691376
50 0.955353915691376
51 0.955353915691376
52 0.955353915691376
53 0.955353915691376
};
\addlegendentry{Centralised ML}
\addplot [thick, color1]
table {%
0 0.49646931886673
1 0.503892838954926
2 0.496107190847397
3 0.503892838954926
4 0.503892838954926
5 0.496107190847397
6 0.672279536724091
7 0.503892838954926
8 0.503892838954926
9 0.504436016082764
10 0.504073858261108
11 0.548795938491821
12 0.504436016082764
13 0.514032244682312
14 0.5102299451828
15 0.514032244682312
16 0.518015563488007
17 0.520550429821014
18 0.52562016248703
19 0.514937520027161
20 0.513126909732819
21 0.514756500720978
22 0.535216391086578
23 0.544269442558289
24 0.536483824253082
25 0.548977017402649
26 0.564729332923889
27 0.566358864307404
28 0.579033136367798
29 0.500995814800262
30 0.602752149105072
31 0.611986219882965
32 0.645482540130615
33 0.707224309444427
34 0.54499363899231
35 0.564729332923889
36 0.705956935882568
37 0.501720070838928
38 0.677349269390106
39 0.706137955188751
40 0.705594778060913
41 0.745428204536438
42 0.737642586231232
43 0.779829800128937
44 0.772225260734558
45 0.723881959915161
46 0.841752648353577
47 0.785985887050629
48 0.817309439182281
49 0.785985887050629
50 0.814231395721436
51 0.808799564838409
52 0.81586092710495
53 0.754481256008148
};
\addlegendentry{BEAS without MULTI-KRUM}
\addplot [thick, color2]
table {%
0 0.496107190847397
1 0.504979193210602
2 0.503892838954926
3 0.519826173782349
4 0.579395234584808
5 0.516023874282837
6 0.561832308769226
7 0.703965246677399
8 0.732935011386871
9 0.727684199810028
10 0.718993306159973
11 0.764258563518524
12 0.797030627727509
13 0.80916166305542
14 0.83161324262619
15 0.847546637058258
16 0.851529955863953
17 0.870360314846039
18 0.881223976612091
19 0.891363382339478
20 0.923230111598969
21 0.9246786236763
22 0.926308155059814
23 0.935542285442352
24 0.93572336435318
25 0.936628639698029
26 0.937533974647522
27 0.947854399681091
28 0.941155195236206
29 0.945862770080566
30 0.949121832847595
31 0.948216557502747
32 0.945138514041901
33 0.941517293453217
34 0.945500612258911
35 0.932826340198517
36 0.939163506031036
37 0.939706683158875
38 0.948578655719757
39 0.949846088886261
40 0.947673380374908
41 0.943871080875397
42 0.948759734630585
43 0.952924132347107
44 0.94948399066925
45 0.950208246707916
46 0.942241549491882
47 0.950932443141937
48 0.94713020324707
49 0.950570344924927
50 0.945319592952728
51 0.950208246707916
52 0.951294600963593
53 0.946405947208405
};
\addlegendentry{BEAS with MULTI-KRUM}
\end{axis}

\end{tikzpicture}


==> figure/reg-acc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color2}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}
\definecolor{color3}{rgb}{0.505882352941176,0.447058823529412,0.698039215686274}
\definecolor{color4}{rgb}{0.8,0.725490196078431,0.454901960784314}
\definecolor{color5}{rgb}{0.392156862745098,0.709803921568627,0.803921568627451}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=None, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=none},
tick align=outside,
tick pos=both,
x grid style={white!80!black},
xlabel={Global Round (s)},
xmajorgrids,
xmin=0, xmax=55,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.5, ymax=1,
ytick style={color=white!15!black}
]
\addplot [thick, color0]
table {%
0 0.955353915691376
1 0.955353915691376
2 0.955353915691376
3 0.955353915691376
4 0.955353915691376
5 0.955353915691376
6 0.955353915691376
7 0.955353915691376
8 0.955353915691376
9 0.955353915691376
10 0.955353915691376
11 0.955353915691376
12 0.955353915691376
13 0.955353915691376
14 0.955353915691376
15 0.955353915691376
16 0.955353915691376
17 0.955353915691376
18 0.955353915691376
19 0.955353915691376
20 0.955353915691376
21 0.955353915691376
22 0.955353915691376
23 0.955353915691376
24 0.955353915691376
25 0.955353915691376
26 0.955353915691376
27 0.955353915691376
28 0.955353915691376
29 0.955353915691376
30 0.955353915691376
31 0.955353915691376
32 0.955353915691376
33 0.955353915691376
34 0.955353915691376
35 0.955353915691376
36 0.955353915691376
37 0.955353915691376
38 0.955353915691376
39 0.955353915691376
40 0.955353915691376
41 0.955353915691376
42 0.955353915691376
43 0.955353915691376
44 0.955353915691376
45 0.955353915691376
46 0.955353915691376
47 0.955353915691376
48 0.955353915691376
49 0.955353915691376
50 0.955353915691376
51 0.955353915691376
52 0.955353915691376
53 0.955353915691376
};
\addlegendentry{Centralised ML}
\addplot [thick, color1]
table {%
0 0.496107190847397
1 0.503892838954926
2 0.503892838954926
3 0.503892838954926
4 0.509505689144135
5 0.496107190847397
6 0.497917801141739
7 0.61904764175415
8 0.661053776741028
9 0.6900235414505
10 0.648560583591461
11 0.741625905036926
12 0.716820597648621
13 0.738366842269897
14 0.753756999969482
15 0.757197201251984
16 0.773492693901062
17 0.768422961235046
18 0.794676780700684
19 0.785261631011963
20 0.797392725944519
21 0.812239706516266
22 0.826181411743164
23 0.854245901107788
24 0.860401928424835
25 0.878145933151245
26 0.889733850955963
27 0.902589201927185
28 0.908383131027222
29 0.911461174488068
30 0.920152068138123
31 0.918703615665436
32 0.92033314704895
33 0.921600580215454
34 0.9246786236763
35 0.920876324176788
36 0.92268693447113
37 0.937171816825867
38 0.930834710597992
39 0.92938619852066
40 0.933550596237183
41 0.938801348209381
42 0.936990737915039
43 0.940611958503723
44 0.934455931186676
45 0.93608546257019
46 0.939344584941864
47 0.938620328903198
48 0.940249860286713
49 0.946768045425415
50 0.940793037414551
51 0.948035478591919
52 0.950932443141937
53 0.950751423835754
};
\addlegendentry{BEAS}
\addplot [thick, color2]
table {%
0 0.503892838954926
1 0.504073858261108
2 0.496107190847397
3 0.528517127037048
4 0.524352729320526
5 0.624479472637177
6 0.662502288818359
7 0.688212931156158
8 0.70106828212738
9 0.719174385070801
10 0.721528172492981
11 0.702516734600067
12 0.770052492618561
13 0.726054668426514
14 0.738728940486908
15 0.805540442466736
16 0.791779816150665
17 0.840847373008728
18 0.846460282802582
19 0.84501177072525
20 0.890277028083801
21 0.902408123016357
22 0.897157371044159
23 0.910555839538574
24 0.91363388299942
25 0.912728607654572
26 0.918341457843781
27 0.92232483625412
28 0.920514225959778
29 0.928843021392822
30 0.92268693447113
31 0.930291533470154
32 0.92938619852066
33 0.926127076148987
34 0.926308155059814
35 0.926127076148987
36 0.93373167514801
37 0.93608546257019
38 0.927756667137146
39 0.945319592952728
40 0.925402879714966
41 0.935180127620697
42 0.94278472661972
43 0.946405947208405
44 0.945138514041901
45 0.940974116325378
46 0.943871080875397
47 0.933550596237183
48 0.938801348209381
49 0.949121832847595
50 0.950027167797089
51 0.936990737915039
52 0.949302911758423
53 0.93608546257019
};
\addlegendentry{BEAS with Backdoor}
\addplot [thick, color3]
table {%
0 0.503892838954926
1 0.496107190847397
2 0.496107190847397
3 0.496107190847397
4 0.503892838954926
5 0.585008144378662
6 0.59858775138855
7 0.506608724594116
8 0.505703449249268
9 0.504617035388947
10 0.5102299451828
11 0.53032773733139
12 0.527792870998383
13 0.510411024093628
14 0.50986784696579
15 0.512402653694153
16 0.515842854976654
17 0.516204953193665
18 0.505703449249268
19 0.514394342899323
20 0.5102299451828
21 0.547528505325317
22 0.558573246002197
23 0.558935344219208
24 0.613615810871124
25 0.58790510892868
26 0.590077877044678
27 0.557305812835693
28 0.584283888339996
29 0.659786343574524
30 0.575592994689941
31 0.636248409748077
32 0.595509707927704
33 0.661234855651855
34 0.696179628372192
35 0.678978800773621
36 0.664493918418884
37 0.684591710567474
38 0.686945497989655
39 0.717725872993469
40 0.703059911727905
41 0.70106828212738
42 0.711931943893433
43 0.725692570209503
44 0.721347093582153
45 0.733659267425537
46 0.746514558792114
47 0.745066106319427
48 0.729313790798187
49 0.781459331512451
50 0.770052492618561
51 0.782545745372772
52 0.792322993278503
53 0.819120049476624
};
\addlegendentry{BEAS with Backdoor + Noise (0.10)}
\addplot [thick, color4]
table {%
0 0.503892838954926
1 0.609089255332947
2 0.496107190847397
3 0.520007252693176
4 0.503892838954926
5 0.600579380989075
6 0.592793762683868
7 0.625203669071198
8 0.651638627052307
9 0.665942430496216
10 0.674814403057098
11 0.68766975402832
12 0.720984995365143
13 0.648379504680634
14 0.712112963199615
15 0.717182695865631
16 0.710121333599091
17 0.743436515331268
18 0.738728940486908
19 0.74289333820343
20 0.789426028728485
21 0.807351052761078
22 0.83559662103653
23 0.841028451919556
24 0.862936794757843
25 0.877783834934235
26 0.850805699825287
27 0.864204227924347
28 0.900597512722015
29 0.90657252073288
30 0.907658874988556
31 0.909831583499908
32 0.903856575489044
33 0.906391441822052
34 0.92667031288147
35 0.925402879714966
36 0.919427871704102
37 0.9246786236763
38 0.928299844264984
39 0.935180127620697
40 0.927394509315491
41 0.92703241109848
42 0.935904383659363
43 0.944233179092407
44 0.933007419109344
45 0.94043093919754
46 0.935904383659363
47 0.937352895736694
48 0.937896072864532
49 0.947854399681091
50 0.938258171081543
51 0.939887762069702
52 0.945681691169739
53 0.938801348209381
};
\addlegendentry{BEAS with Backdoor + Prune Sparcity (0.50)}
\addplot [thick, color5]
table {%
0 0.504073858261108
1 0.503711760044098
2 0.496107190847397
3 0.504254937171936
4 0.622125685214996
5 0.589715719223022
6 0.591707408428192
7 0.592612683773041
8 0.617599129676819
9 0.617961227893829
10 0.629549145698547
11 0.664674997329712
12 0.657794654369354
13 0.691109895706177
14 0.70903491973877
15 0.725330412387848
16 0.71808797121048
17 0.734564542770386
18 0.728046357631683
19 0.748687326908112
20 0.772406280040741
21 0.823646545410156
22 0.837769329547882
23 0.849719345569611
24 0.843563258647919
25 0.868911802768707
26 0.877421677112579
27 0.889733850955963
28 0.884845197200775
29 0.900778591632843
30 0.915082395076752
31 0.916168749332428
32 0.915806651115417
33 0.913452804088593
34 0.928480923175812
35 0.929929375648499
36 0.923049092292786
37 0.936990737915039
38 0.940249860286713
39 0.944233179092407
40 0.944957435131073
41 0.935542285442352
42 0.939525604248047
43 0.943871080875397
44 0.944595336914062
45 0.946043789386749
46 0.949846088886261
47 0.948940813541412
48 0.940249860286713
49 0.946405947208405
50 0.948035478591919
51 0.944414258003235
52 0.951294600963593
53 0.952199876308441
};
\addlegendentry{BEAS with Backdoor + Clip (0.60)}
\end{axis}

\end{tikzpicture}

